Coupling between risk and cautious behavior affect epidemic morbidity, mortality and dynamics

Models for epidemic spread typically account for variable risk factors but do not account for the correlation between behavior and risk. Here we extend these models to account for such correlations. We find that a positive correlation between behavior and risk, i.e., voluntary risk aversion by individuals at high risk and risk-taking behavior by individuals at low risk, leads to a linear reduction in morbidity and mortality and load on healthcare services compared to the uncorrelated case. We show that increasing caution in response to news from countries with a preceding outbreak leads to a more graded response to a lock-down. We also show that if vaccinated individuals are less cautious an increase in herd immunity threshold ensues.

==> newFigs/name.tex <==
(Resolved Components Analysis, [1]) aims at characterizing globally a space-variant PSFs field. Given a set of aliased and noisy images of unresolved objects (stars images from a telescope for instance), RCA estimates well-resolved and noise-free PSFs at the observations positions, in particular, exploiting the spatial correlation of the PSFs across the imaging system field of view (FOV). Let consider a set of p images of unresolved objects $$\mathbf{y}_1,\dots,\mathbf{y}_p$$ in a given instrument FOV and $$\mathbf{x}_1,\dots,\mathbf{x}_p$$ the corresponding ideal PSFs; these images are treated as column vectors and we note $$\mathbf{Y} = [\mathbf{y}_1,\dots,\mathbf{y}_p]$$ and $$\mathbf{X} = [\mathbf{x}_1,\dots,\mathbf{x}_p]$$. RCA minimizes $$ \frac{1}{2}{\|\mathbf{Y}-\mathcal{F}(\mathbf{X})\|_F^2}$$, where $$\mathcal{F}$$ accounts for the observed stars downsampling; this is done subject to several constraints over $$\mathbf{X}$$:

Positivity constraint: each PSF $$\mathbf{x}_j$$ should be positive;
Low rank constraint: each estimated PSF is forced to be a linear combination of a few number esimated of "eigen" PSFs; $$\mathbf{x}_j = \sum_{i=1}^r a_{ij} \mathbf{s}_i$$, with $$r \ll p$$ or equivalently, $$\mathbf{X} = \mathbf{S}\mathbf{A}$$, $$\mathbf{S}$$ and $$\mathbf{A}$$ being low rank matrices;
Piece-wise smoothness constraint: we can assume that the vectors $$\mathbf{x}_j$$ are structured; promoting the sparsity of the "eigen" PSFs $$\mathbf{s}_j$$ in an appropriate dictionary $$\boldsymbol{\Phi}$$ allows to capture the spatial correlations within the PSFs themselves;
Proximity constraints: the more two PSFs are close in the FOV, the more they should be similar; the p values relative to the $$i^{th}$$ line of $$\mathbf{A}$$ correspond to the contribution of the $$i^{th}$$ "eigen" PSF across the field of view; therefore the PSFs field regularity is enforced by constraining $$\mathbf{A}$$'s lines; specifically, each line is calculated as a sparse linear combination of spatial frequencies atoms: $$\mathbf{A} = \boldsymbol{\alpha}\mathbf{U}^T$$ 
